Compact Trip Representation over Networks

We present a new Compact Trip Representation (CTR) that allows us to manage users' trips (moving objects) over networks. These could be public transportation networks (buses, subway, trains, and so on) where nodes are stations or stops, or road networks where nodes are intersections. CTR represents the sequences of nodes and time instants in users' trips. The spatial component is handled with a data structure based on the well-known Compressed Suffix Array (CSA), which provides both a compact representation and interesting indexing capabilities. We also represent the temporal component of the trips, that is, the time instants when users visit nodes in their trips. We create a sequence with these time instants, which are then self-indexed with a balanced Wavelet Matrix (WM). This gives us the ability to solve range-interval queries efficiently. We show how CTR can solve relevant spatial and spatio-temporal queries over large sets of trajectories. Finally, we also provide experimental results to show the space requirements and query efficiency of CTR.

==> Makefile <==
all:  pdf open

open:
	gnome-open paper.pdf &

pdf:
	latex paper.tex
	bibtex paper
	latex paper.tex
	latex paper.tex
	dvips paper.dvi
	ps2pdf paper.ps
	#dvipdfm paper.dvi
	rm -f paper.blg
	rm -f paper.aux
	#rm -f paper.bbl
	rm -f paper.log
	#rm -f paper.dvi
	rm -f paper.ps

diff:
	latexdiff paper_last.tex paper.tex > paper_diff.tex
	latex paper_diff.tex
	latex paper_diff.tex
	bibtex paper_diff
	latex paper_diff.tex
	latex paper_diff.tex
	dvips paper_diff.dvi
	ps2pdf paper_diff.ps
	rm -f paper_diff.blg
	rm -f paper_diff.aux
	rm -f paper_diff.bbl
	rm -f paper_diff.log
	rm -f paper_diff.ps

clean:
	#dos2unix *.tex
	rm -f paper.dvi
	rm -f paper.ps
	#rm -f paper.pdf
	rm -f paper_diff*

##images:
##	cd figures && pdftops -eps *.pdf && cd ..

tar:
#	rm -f dcc2015.tar.gz
#	tar czvf dcc2015.tar.gz figures paper_last.tex \
#			 paper.tex *.bib Makefile
	rm -f spire2016.7z
	7z a spire2016.7z llncs.cls figures *.tex *.bib Makefile

zip:
	rm -f spire2016.zip
	zip -r spire2016.zip *

